R3DPA: Leveraging 3D Representation Alignment and RGB Pretrained Priors for LiDAR Scene Generation

LiDAR scene synthesis is an emerging solution to scarcity in 3D data for robotic tasks such as autonomous driving. Recent approaches employ diffusion or flow matching models to generate realistic scenes, but 3D data remains limited compared to RGB datasets with millions of samples. We introduce R3DPA, the first LiDAR scene generation method to unlock image-pretrained priors for LiDAR point clouds, and leverage self-supervised 3D representations for state-of-the-art results. Specifically, we (i) align intermediate features of our generative model with self-supervised 3D features, which substantially improves generation quality; (ii) transfer knowledge from large-scale image-pretrained generative models to LiDAR generation, mitigating limited LiDAR datasets; and (iii) enable point cloud control at inference for object inpainting and scene mixing with solely an unconditional model. On the KITTI-360 benchmark R3DPA achieves state of the art performance. Code and pretrained models are available at https://github.com/valeoai/R3DPA.

==> tables/evaluation_on_trainval.tex <==
    \begin{table*}[htbp]
\centering
\small
\begin{tabular}{lcccccccc}
\toprule
Method & FRID & FLD & FSVD & FPVD & JSD & TV & MMD \\ \\
 & $\times 10^{0}$ & $\times 10^{-1}$ & $\times 10^{0}$ & $\times 10^{0}$ & $\times 10^{-2}$ & $\times 10^{-2}$ & $\times 10^{-5}$ \\
\midrule
UltraLiDAR & - & - & 71.690 & 64.780 & 74.720 & 180.500 & 123.300 \\
\midrule
LiDM & 42.310 & 9.515 & 16.540 & 17.600 & 18.870 & 35.640 & 11.320 \\
\midrule
R2DM & 9.844 & 4.044 & \underline{10.990} & \underline{11.990} & \underline{4.967} & \underline{7.185} & \underline{8.502} \\
\midrule
R2Flow & \underline{3.885} & \underline{3.819} & 18.480 & 18.530 & 5.171 & 8.081 & \textbf{7.844} \\
\midrule
\textbf{\ours} (ours) & \textbf{2.159} & \textbf{2.697} & \textbf{6.810} & \textbf{8.336} & \textbf{4.599} & \textbf{6.940} & 8.870 \\
\bottomrule
\end{tabular}
\caption{Combined evaluation results across models on trainval}
\label{tab:combined_results}
\end{table*}


==> tables/evaluation_on_valonly.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{lcccccccc}
\toprule
Method & FRD & FRID & FLD & FSVD & FPVD & JSD & TV & MMD \\ \\
 & $\times 10^{0}$ & $\times 10^{0}$ & $\times 10^{-1}$ & $\times 10^{0}$ & $\times 10^{0}$ & $\times 10^{-2}$ & $\times 10^{-2}$ & $\times 10^{-5}$ \\
\midrule
UltraLiDAR & - & - & - & 73.590 & 65.830 & 74.720 & 180.500 & 123.300 \\
\midrule
LiDM temp & - & 47.330 & 10.190 & 16.010 & 17.360 & 19.170 & 36.170 & 11.320 \\
\midrule
R2DM & \underline{9.542} & 15.540 & \underline{7.889} & \underline{12.670} & \underline{13.210} & \textbf{5.775} & \textbf{9.346} & 8.502 \\
\midrule
R2Flow & \textbf{8.912} & \underline{8.874} & 8.357 & 20.800 & 20.270 & \underline{5.974} & \underline{10.220} & \textbf{7.844} \\
\midrule
UNet 800k & - & \textbf{8.023} & \textbf{6.877} & \textbf{8.745} & \textbf{9.378} & 5.984 & 10.690 & \underline{8.416} \\
\bottomrule
\end{tabular}
\caption{Combined evaluation results across models on valonly}
\label{tab:combined_results}
\end{table*}
